Impact of instrument and data characteristics in the interferometric reconstruction of the 21 cm power spectrum

Combining the visibilities measured by an interferometer to form a cosmological power spectrum is a complicated process. In a delay-based analysis, the mapping between instrumental and cosmological space is not a one-to-one relation. Instead, neighbouring modes contribute to the power measured at one point, with their respective contributions encoded in the window functions. To better understand the power measured by an interferometer, we assess the impact of instrument characteristics and analysis choices on these window functions. Focusing on the Hydrogen Epoch of Reionization Array (HERA) as a case study, we find that long-baseline observations correspond to enhanced low-k tails of the window functions, which facilitate foreground leakage, whilst an informed choice of bandwidth and frequency taper can reduce said tails. With simple test cases and realistic simulations, we show that, apart from tracing mode mixing, the window functions help accurately reconstruct the power spectrum estimator of simulated visibilities. The window functions depend strongly on the beam chromaticity, and less on its spatial structure - a Gaussian approximation, ignoring side lobes, is sufficient. Finally, we investigate the potential of asymmetric window functions, down-weighting the contribution of low-k power to avoid foreground leakage. The window functions presented here correspond to the latest HERA upper limits for the full Phase I data. They allow an accurate reconstruction of the power spectrum measured by the instrument and will be used in future analyses to confront theoretical models and data directly in cylindrical space.

==> Exact window functions/author-list.tex <==
\author[A. Gorce et al.]{	Adélie  Gorce$^{1}$\thanks{Email: \href{mailto:adelie.gorce@mcgill.ca}{adelie.gorce@mcgill.ca}},
	Samskruthi  Ganjam$^{1}$,
	Adrian  Liu$^{1}$,
	Steven G. Murray$^{2}$,
	Zara  Abdurashidova$^{3}$,
	Tyrone  
\newauthor
	Adams$^{4}$,
	James E. Aguirre$^{5}$,
	Paul  Alexander$^{6}$,
	Zaki S. Ali$^{3}$,
	Rushelle  Baartman$^{4}$,
	Yanga  Balfour$^{4}$,
	Adam 
\newauthor
	P. Beardsley$^{2,7,\dagger}$,
	Gianni  Bernardi$^{8,9,4}$,
	Tashalee S. Billings$^{5}$,
	Judd D. Bowman$^{2}$,
	Richard F. Bradley$^{10}$,
\newauthor
	Philip  Bull$^{11,12}$,
	Jacob  Burba$^{13}$,
	Steven  Carey$^{6}$,
	Chris L. Carilli$^{14}$,
	Carina  Cheng$^{3}$,
	David R. DeBoer$^{15}$,
\newauthor
	Eloy  de~Lera~Acedo$^{6}$,
	Matt  Dexter$^{15}$,
	Joshua S. Dillon$^{3}$,
	Nico  Eksteen$^{4}$,
	John  Ely$^{6}$,
	Aaron  Ewall-Wice$^{3,16}$,
\newauthor
	Nicolas  Fagnoni$^{6}$,
	Randall  Fritz$^{4}$,
	Steven R. Furlanetto$^{17}$,
	Kingsley  Gale-Sides$^{6}$,
	Brian  Glendenning$^{18}$,
\newauthor
	Deepthi  Gorthi$^{3}$,
	Bradley  Greig$^{19}$,
	Jasper  Grobbelaar$^{4}$,
	Ziyaad  Halday$^{4}$,
	Bryna J. Hazelton$^{20,21}$,
\newauthor
    Jacqueline N. Hewitt$^{22,23}$,
	Jack  Hickish$^{15}$,
	Daniel C. Jacobs$^{2}$,
	Austin  Julius$^{4}$,
	MacCalvin  Kariseb$^{4}$,
\newauthor
	Nicholas S. Kern$^{3,23}$,
	Joshua  Kerrigan$^{13}$,
	Piyanat  Kittiwisit$^{12}$,
	Saul A. Kohn$^{5}$,
	Matthew  Kolopanis$^{2}$,
\newauthor
	Adam  Lanman$^{1}$,
	Paul  La~Plante$^{3,24,25}$,
	Anita  Loots$^{4}$,
	David Harold~Edward MacMahon$^{15}$,
	Lourence 
\newauthor
    Malan$^{4}$,
	Cresshim  Malgas$^{4}$,
	Keith  Malgas$^{4}$,
	Bradley  Marero$^{4}$,
	Zachary E. Martinot$^{5}$,
	Andrei  Mesinger$^{26}$,
\newauthor
	Mathakane  Molewa$^{4}$,
	Miguel F. Morales$^{20}$,
	Tshegofalang  Mosiane$^{4}$,
	Abraham R. Neben$^{23}$,
	Bojan
\newauthor
    Nikolic$^{6}$,
	Hans  Nuwegeld$^{4}$,
	Aaron R. Parsons$^{3}$,
	Nipanjana  Patra$^{3}$,
	Samantha  Pieterse$^{4}$,
	Jonathan C. 
\newauthor
    Pober$^{13}$,
	Nima  Razavi-Ghods$^{6}$,
	James  Robnett$^{14}$,
	Kathryn  Rosie$^{4}$,
	Peter  Sims$^{1}$,
	Hilton  Swarts$^{4}$,
\newauthor
	Nithyanandan  Thyagarajan$^{27,14}$,
	Pieter  van~Wyngaarden$^{4}$,
	Peter K.~G. Williams$^{28,29}$,
	Haoxuan  Zheng$^{23}$
\\
$^{1}$ Department of Physics and McGill Space Institute, McGill University, 3600 University Street, Montreal, QC H3A 2T8, Canada\\
$^{2}$ School of Earth and Space Exploration, Arizona State University, Tempe, AZ 85287-1404, USA\\
$^{3}$ Department of Astronomy, University of California, Berkeley, CA 94720-3411, USA\\
$^{4}$ South African Radio Astronomy Observatory, Black River Park, 2 Fir Street, Observatory, Cape Town, 7925, South Africa\\
$^{5}$ Department of Physics and Astronomy, University of Pennsylvania, Philadelphia, PA 19104-6396, USA\\
$^{6}$ Cavendish Astrophysics, University of Cambridge, Cambridge CB3 0HE, UK\\
$^{7}$ Department of Physics, Winona State University, Winona, MN 55987, USA\\
$^{\dagger}$ NSF Astronomy and Astrophysics Postdoctoral Fellow\\
$^{8}$ INAF-Istituto di Radioastronomia, via Gobetti 101, 40129 Bologna, Italy\\
$^{9}$ Department of Physics and Electronics, Rhodes University, PO Box 94, Grahamstown, 6140, South Africa\\
$^{10}$ National Radio Astronomy Observatory, Charlottesville, VA 22903, USA\\
$^{11}$ Jodrell Bank Centre for Astrophysics, University of Manchester, Manchester, M13 9PL, UK\\
$^{12}$ Department of Physics and Astronomy,  University of Western Cape, Cape Town, 7535, South Africa\\
$^{13}$ Department of Physics, Brown University, Providence, RI 02906, USA\\
$^{14}$ National Radio Astronomy Observatory, Socorro, NM 87801, USA\\
$^{15}$ Radio Astronomy Lab, University of California, Berkeley, CA 94720-3411, USA\\
$^{16}$ Department of Physics, University of California, Berkeley, CA 94720-3411, USA\\
$^{17}$ Department of Physics and Astronomy, University of California, Los Angeles, CA 90095-1547, USA\\
$^{18}$ National Radio Astronomy Observatory, Socorro, NM 87801-0387, USA\\
$^{19}$ School of Physics, University of Melbourne, Parkville, VIC 3010, Australia\\
$^{20}$ Department of Physics, University of Washington, Seattle, WA 98195-1560, USA\\
$^{21}$ eScience Institute, University of Washington, Seattle, WA 98195-1560, USA\\
$^{22}$ MIT Kavli Institute, Massachusetts Institute of Technology, Cambridge, MA 02139, USA\\
$^{23}$ Department of Physics, Massachusetts Institute of Technology, Cambridge, MA 02142, USA\\
$^{24}$ Department of Computer Science, University of Nevada, Las Vegas, NV 89154, USA\\
$^{25}$ Nevada Center for Astrophysics, University of Nevada, Las Vegas, NV 89154, USA\\
$^{26}$ Scuola Normale Superiore, 56126 Pisa, Italy\\
$^{27}$ Commonwealth Scientific and Industrial Research Organisation (CSIRO), Space \& Astronomy, P. O. Box 1130, Bentley, WA 6102, Australia\\
$^{28}$ Center for Astrophysics, Harvard \& Smithsonian, Cambridge, MA 02138, USA\\
$^{29}$ American Astronomical Society, Washington, DC 20006, USA
\vspace{3cm}
}

